Multimodal Difference Learning for Sequential Recommendation

Sequential recommendations have drawn significant attention in modeling the user's historical behaviors to predict the next item. With the booming development of multimodal data (e.g., image, text) on internet platforms, sequential recommendation also benefits from the incorporation of multimodal data. Most methods introduce modal features of items as side information and simply concatenates them to learn unified user interests. Nevertheless, these methods encounter the limitation in modeling multimodal differences. We argue that user interests and item relationships vary across different modalities. To address this problem, we propose a novel Multimodal Difference Learning framework for Sequential Recommendation, MDSRec for brevity. Specifically, we first explore the differences in item relationships by constructing modal-aware item relation graphs with behavior signal to enhance item representations. Then, to capture the differences in user interests across modalities, we design a interest-centralized attention mechanism to independently model user sequence representations in different modalities. Finally, we fuse the user embeddings from multiple modalities to achieve accurate item recommendation. Experimental results on five real-world datasets demonstrate the superiority of MDSRec over state-of-the-art baselines and the efficacy of multimodal difference learning.

==> section/checklist.tex <==

% !TEX spellcheck = en_US
% !TeX root = ./main.tex
\paragraph{This paper:}
\begin{itemize}
	\item Includes a conceptual outline and/or pseudocode description of AI methods introduced (yes/partial/no/NA) {\bf yes}
	\item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (yes/no){\bf yes}
	\item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper (yes/no){\bf yes}
\end{itemize}
\paragraph{Does this paper make theoretical contributions? (yes/no)}{\bf yes}

If yes, please complete the list below.
\begin{itemize}
	\item All assumptions and restrictions are stated clearly and formally. (yes/partial/no){\bf yes}
	\item All novel claims are stated formally (e.g., in theorem statements). (yes/partial/no){\bf yes}
	\item Proofs of all novel claims are included. (yes/partial/no){\bf yes}
	\item Proof sketches or intuitions are given for complex and/or novel results. (yes/partial/no){\bf yes}
	\item Appropriate citations to theoretical tools used are given. (yes/partial/no){\bf yes}
	\item All theoretical claims are demonstrated empirically to hold. (yes/partial/no/NA){\bf yes}
	\item All experimental code used to eliminate or disprove claims is included. (yes/no/NA){\bf yes}
\end{itemize}
\paragraph{Does this paper rely on one or more datasets? (yes/no)}{\bf yes}

If yes, please complete the list below.
\begin{itemize}
	\item A motivation is given for why the experiments are conducted on the selected datasets (yes/partial/no/NA){\bf yes}
	\item All novel datasets introduced in this paper are included in a data appendix. (yes/partial/no/NA){\bf NA}
	\item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no/NA){\bf NA}
	\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (yes/no/NA){\bf yes}
	\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (yes/partial/no/NA){\bf yes}
	\item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (yes/partial/no/NA){\bf yes}
\end{itemize}
\paragraph{Does this paper rely on one or more datasets? (yes/no)}{\bf yes}

If yes, please complete the list below.
\begin{itemize}
	\item Any code required for pre-processing data is included in the appendix. (yes/partial/no).{\bf yes}
	\item All source code required for conducting and analyzing the experiments is included in a code appendix. (yes/partial/no){\bf yes}
	\item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no){\bf yes}
	\item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (yes/partial/no){\bf partial}
	\item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes/partial/no/NA){\bf yes}
	\item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (yes/partial/no){\bf partial}
	\item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (yes/partial/no){\bf yes}
	\item This paper states the number of algorithm runs used to compute each reported result. (yes/no){\bf yes}
	\item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (yes/no){\bf yes}
	\item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes/partial/no){\bf yes}
	\item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (yes/partial/no/NA){\bf partial}
	\item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (yes/partial/no/NA){\bf partial}
	
\end{itemize}


